Boosting Monocular Depth Estimation Models to High-Resolution via Content-Adaptive Multi-Resolution Merging

Neural networks have shown great abilities in estimating depth from a single image. However, the inferred depth maps are well below one-megapixel resolution and often lack fine-grained details, which limits their practicality. Our method builds on our analysis on how the input resolution and the scene structure affects depth estimation performance. We demonstrate that there is a trade-off between a consistent scene structure and the high-frequency details, and merge low- and high-resolution estimations to take advantage of this duality using a simple depth merging network. We present a double estimation method that improves the whole-image depth estimation and a patch selection method that adds local details to the final result. We demonstrate that by merging estimations at different resolutions with changing context, we can generate multi-megapixel depth maps with a high level of detail using a pre-trained model.

==> images/depth_refinementmethods.tex <==
% \begin{table}[t]
% \caption{
%     depth refinement methods comparison
% }
% \resizebox{\linewidth}{!}
% {
% {\setlength{\extrarowheight}{4pt}
% \setlength\arrayrulewidth{1pt}
% % \rowcolors{2}{gray!25}{}
% \begin{tabular}{|l|l|l|llll|}
%     \arrayrulecolor{gray!25}\hline 
%     dataset                       & network                 & method & ord~\cite{xian2020sgr} & ddr(ours) & rmse & $\delta>1.25$  \\
%     \arrayrulecolor{gray!25}\hline 
%     \multirow{9}{*}{Middleburry} & \multirow{3}{*}{MiDaS}   & - & - & - & - & - \\
%                                  &                          & - & - & - & - & - \\
%                                  &                          & - & - & - & - & - \\
%                                  & \multirow{3}{*}{SGR}   & - & - & - & - & - \\
%                                  &                          & - & - & - & - & - \\
%                                  &                          & - & - & - & - & - \\
%                                  & \multirow{3}{*}{Megadepth}   & - & - & - & - & - \\
%                                  &                          & - & - & - & - & - \\
%                                  &                          & - & - & - & - & - \\
%     \arrayrulecolor{gray!25}\hline 

                           
% \end{tabular}
% }
% }
% \negvspace
% \negvspace
% \label{tab:depth_refinement}
% \end{table}


==> images/our_performance_backup.tex <==
\begin{table}[t]
\caption{
    Comparison on Middleburry2014 \cite{Scharstein2014HighResolutionSD}. Baselines: MiDas and SGR 
}
\resizebox{\linewidth}{!}
{
{\setlength{\extrarowheight}{4pt}
\setlength\arrayrulewidth{1pt}
\begin{tabular}{|l|l|llll||l|l|llll|}
    \arrayrulecolor{gray!25}\hline 
                                  & Method & ORD~\cite{xian2020sgr} & DDR (ours) & RMSE & $\delta>1.25$  \\
    \arrayrulecolor{gray!25}\hline 
                                  \parbox[t]{2mm}{\multirow{6}{*}{\rotatebox[origin=c]{90}{MiDaS~\cite{midas}}}}  
                                  & MiDas                             & 0.3840 & 0.3343 & 0.1708 & 0.7649 \\ 
                                  & Refinement-Bilateral                & 0.3806 & 0.3366 & 0.1707 & 0.7627 \\ 
                                  & Refinement-3DKenBurns               & 0.3826 & 0.3377 & 0.1704 & 0.7622 \\  \cline{2-6} 
                                  & Single-estimation (t=0 \%)                      & 0.3554 & 0.2504 & \textbf{0.1481} & \textbf{0.7161} \\  
                                  & Double-estimation (t=20\%)                     & 0.3496 & 0.1709 & 0.1563 & 0.7364 \\\cline{2-6} 
                                  & OURS                                & \textbf{0.3467} & \textbf{0.1578} & 0.1557 & 0.7406 \\ 
    \arrayrulecolor{gray!25}\hline 
    \arrayrulecolor{gray!25}\hline 
                                   \parbox[t]{2mm}{\multirow{6}{*}{\rotatebox[origin=c]{90}{SGR~\cite{xian2020sgr}}}}     
                                   & SGR                                 & 0.4087 & 0.3889 & 0.2123 & 0.7989 \\  
                                   & Refinement-Bilateral                & 0.4078 & 0.3904 & 0.2122 & 0.7990 \\ 
                                   & Refinement-3DKenBurns               & 0.4081 & 0.3880 & 0.2115 & 0.7993 \\  \cline{2-6} 
                                   & Single-estimation (t=0 \%)          & 0.4312 & 0.3131 & 0.1999 & \textbf{0.7841} \\  
                                   & Double-estimation (t=20\%)          & 0.3944 & 0.2540 & 0.1983 & 0.7931 \\\cline{2-6} 
                                   & OURS                                & \textbf{0.3879} & \textbf{0.2324} & \textbf{0.1973} & 0.7891 \\
    \arrayrulecolor{gray!25}\hline 

\end{tabular}
}
}
\negvspace
\negvspace
\label{tab:depth_estimation_performance1}
\end{table}


\begin{table}[t]
\caption{
    Comparison on Ibims-1. 
}
\resizebox{\linewidth}{!}
{
{\setlength{\extrarowheight}{4pt}
\setlength\arrayrulewidth{1pt}
% \rowcolors{2}{gray!25}{}
\begin{tabular}{|l|l|llll|}
    \arrayrulecolor{gray!25}\hline 
                                  & Method & ORD~\cite{xian2020sgr} & DDR (ours) & RMSE & $\delta>1.25$  \\
    \arrayrulecolor{gray!25}\hline 
                                  \parbox[t]{2mm}{\multirow{6}{*}{\rotatebox[origin=c]{90}{MiDaS~\cite{midas}}}}  
                                  & MiDaS                             & 0.4002 & 0.3698 & \textbf{0.1596} & \textbf{0.6345} \\  
                                  & Refinement-Bilateral                & 0.3982 & 0.3768 & 0.1596 & 0.6350 \\  
                                  & Refinement-3DKenBurns               & 0.4006 & 0.3761 & 0.1600 & 0.6351 \\ \cline{2-6} 
                                  & Single-estimation (t=0 \%)        & 0.4504 & 0.3269 & 0.1687 & 0.6633 \\  
                                  & Double-estimation (t=20\%)        & 0.4112 & 0.3272 & 0.1597 & 0.6386 \\\cline{2-6} 
                                  & OURS                                & \textbf{0.3938} & \textbf{0.3222} & 0.1598 & 0.6390 \\
   \arrayrulecolor{gray!25}\hline 
   \arrayrulecolor{gray!25}\hline 
                                  \parbox[t]{2mm}{\multirow{6}{*}{\rotatebox[origin=c]{90}{SGR~\cite{xian2020sgr}}}}   
                                  & SGR                             & 0.5555 & 0.4736 & 0.1956 & 0.7513 \\  
                                  & Refinement-Bilateral                & 0.5551 & 0.4750 & 0.1956 & 0.7501 \\  
                                  & Refinement-3DKenBurns               & 0.5488 & 0.4780 & \textbf{0.1953} & 0.7482 \\\cline{2-6} 
                                  & Single-estimation (t=0 \%)         & 0.6343 & 0.4901 & 0.2146 & 0.7856 \\  
                                  & Double-estimation (t=20\%)       & 0.5591 & 0.4829 & 0.1967 & 0.7473 \\\cline{2-6} 
                                  & OURS                                & \textbf{0.5538} & \textbf{0.4671} & 0.1965 & \textbf{0.7460} \\ 
    \arrayrulecolor{gray!25}\hline 

\end{tabular}
}
}
\negvspace
\negvspace
\label{tab:depth_estimation_performance2}
\end{table}


==> images/stateoftheart_old.tex <==
\begin{table*}[t]
\caption{
    state of the art comparison on the Middlebury dataset~\cite{Scharstein2014HighResolutionSD}
}
\resizebox{\linewidth}{!}
{
{\setlength{\extrarowheight}{4pt}
\setlength\arrayrulewidth{1pt}
\rowcolors{2}{gray!25}{}
\begin{tabular}
{|cc!{\color{gray!25}\vrule}ccccccccccc|}
    \arrayrulecolor{gray!25}\hline 
    \multicolumn{2}{!{\color{gray!25}\vrule}c!{\color{gray!25}\vrule} }{Method} &
    ord~\cite{xian2020sgr} & ddr(ours) & rmse & $\delta>1.25$ & $\delta>1.25^2$ & $\delta>1.25^3$ & $log_{10}$ & absrel & sqrel & Rank
    \\
    Method & Network &&&&&&&&
    \\
    Vanilla & MiDaS~\cite{midas} & 0.3840 & 0.3343 & 0.1708 & 0.7649 & 0.5392 & 0.3587 & 0.2810 & 0.7242 & 0.1042 & -
    \\
    global adaptive base & MiDaS & 0.3496 & 0.1709 & 0.1563 & 0.7364 & 0.5086 & 0.3316 & 0.2576 & 0.6540 & 0.0936 & -
    \\
    Pipeline & MiDaS & 0.3467 & 0.1578 & 0.1557 & 0.7406 & 0.5111 & 0.3377 & 0.2586 & 0.6676 & 0.1014 & -
    \\
    Pipeline (only single estimation) & MiDaS & 0.3535 & 0.1744 & 0.1606 & 0.7512 & 0.5201 & 0.3500 & 0.2669 & 0.6918 & 0.1103 & -
    \\
    Pipeline (only smaller half of crops) & MiDaS & 0.3499 & 0.1576 & 0.1560 & 0.7402 & 0.5135 & 0.3378 & 0.2583 & 0.6653 & 0.1007 & -
    \\
    Depth Displacement ~\cite{Ramamonjisoa_2020_CVPR} & MiDaS & 0.3842 & 0.3867 & 0.1692 & 0.7717 & 0.5321 & 0.3552 & 0.2774 & 0.7394 & 0.1025 & -

    % Vanilla & SGR~\cite{xian2020sgr} & - & - & - & - & - & - & - & - & - & -
    % \\
    % global adaptive base & SGR~\cite{xian2020sgr} & - & - & - & - & - & - & - & - & - & -
    % \\
    % Pipeline & SGR~\cite{xian2020sgr} & - & - & - & - & - & - & - & - & - & -
    % \\
    % Vanilla & Megadepth~\cite{li2018megadepth} & - & - & - & - & - & - & - & - & - & -
    % \\
    % global adaptive base & Megadepth~\cite{li2018megadepth} & - & - & - & - & - & - & - & - & - & -
    % \\
    % Pipeline & Megadepth~\cite{li2018megadepth} & - & - & - & - & - & - & - & - & - & -
    % \\
    \\
    \arrayrulecolor{gray!25}\hline

\end{tabular}
}

}
\negvspace
\negvspace
\label{tab:doubleest}
\end{table*}






\begin{table*}[t]
\caption{
    state of the art comparison on the Ibims1 dataset~\cite{Koch18}
}
\resizebox{\linewidth}{!}
{
{\setlength{\extrarowheight}{4pt}
\setlength\arrayrulewidth{1pt}
\rowcolors{2}{gray!25}{}
\begin{tabular}
{|cc!{\color{gray!25}\vrule}ccccccccccc|}
    \arrayrulecolor{gray!25}\hline 
    \multicolumn{2}{!{\color{gray!25}\vrule}c!{\color{gray!25}\vrule} }{Method} &
    ord~\cite{xian2020sgr} & ddr(ours) & rmse & $\delta>1.25$ & $\delta>1.25^2$ & $\delta>1.25^3$ & $log_{10}$ & absrel & sqrel & Rank
    \\
    Method & Network &&&&&&&&
    \\
    Vanilla & MiDaS~\cite{midas} & 0.4022 & 0.3698 & 0.1596 & 0.6345 & 0.4127 & 0.2712 & 0.2473 & 2.0325 & 0.7903 & -
    \\
    global adaptive base & MiDaS & 0.4006 & 0.3272 & 0.1597 & 0.6386 & 0.4139 & 0.2716 & 0.2474 & 2.0449 & 0.7943 & -
    \\
    Pipeline & MiDaS & 0.4044 & 0.3212 & 0.1600 & 0.6393 & 0.4153 & 0.2724 & 0.2478 & 2.0511 & 0.8007 & -
    \\
    Depth Displacement ~\cite{Ramamonjisoa_2020_CVPR} & MiDaS & 0.4107 & 0.4359 & 0.1603 & 0.6384 & 0.4159 & 0.2738 & 0.2488 & 2.0657 & 0.7952 & -

    % Vanilla & SGR~\cite{xian2020sgr} & - & - & - & - & - & - & - & - & - & -
    % \\
    % global adaptive base & SGR~\cite{xian2020sgr} & - & - & - & - & - & - & - & - & - & -
    % \\
    % Pipeline & SGR~\cite{xian2020sgr} & - & - & - & - & - & - & - & - & - & -
    % \\
    % Vanilla & Megadepth~\cite{li2018megadepth} & - & - & - & - & - & - & - & - & - & -
    % \\
    % global adaptive base & Megadepth~\cite{li2018megadepth} & - & - & - & - & - & - & - & - & - & -
    % \\
    % Pipeline & Megadepth~\cite{li2018megadepth} & - & - & - & - & - & - & - & - & - & -
    % \\
    \\
    \arrayrulecolor{gray!25}\hline

\end{tabular}
}

}
\negvspace
\negvspace
\label{tab:doubleest}
\end{table*}

==> imagetex/contextsize.tex <==
\begin{figure*}
\showimagew[0.5\linewidth]{images/fourier}
\caption{
Effect of context - 1. row - amount: center crop with two insets + 4 crops with increasing context size
2. row - resolution: full depth estimation, two insets + 4 higher midas sizes
3. row - density: three crops, 1. too low density, 2. optimal density, 3. too high density
\negvspace
}
\label{fig:contextsize}
\end{figure*}

==> imagetex/cropcontext.tex <==
\begin{figure}
\showimagew[\linewidth]{images/cropcontext}
\caption{
Two crops at same sizes with changing amount of context
\negvspace
}
\label{fig:cropcontext}
\end{figure}

==> imagetex/cropoverview.tex <==
\begin{figure*}
\showimagew[0.5\linewidth]{images/fourier}
\caption{
Example of the crops our method is selecting: color indicates cropsize.
\negvspace
}
\label{fig:cropoverview}
\end{figure*}

==> imagetex/introanalysis.tex <==
\begin{figure*}
\showimagew[0.35\linewidth]{images/fourier}
\caption{
Different input resolutions and different crops for the image in teaser, with detailed explanations on why they fail (not enough context, receptive size etc.) in this caption
\negvspace
}
\label{fig:introanalysis}
\end{figure*}

==> imagetex/oraclemidas.tex <==
\begin{figure*}
\showimagew[0.5\linewidth]{images/fourier}
\caption{
Performance comparison: MiDas, OracleMiDas, Ours
\negvspace
}
\label{fig:oracle}
\end{figure*}

==> tex/intro_orig.tex <==
% !TEX root = ../depth.tex

Monocular depth estimation aims at extracting the structure of the scene from a single image.
Unlike multi-camera depth estimation approaches such as depth from stereo or multi-view stereo, which utilize low-level depth cue disparity, or depth from video approaches such as SLAM that also use motion parallax, monocular depth estimation has to rely on higher-level cues.
These cues come from relative size of objects, changing behavior of texture gradients depending on depth and perspective, foreground objects occluding the background, and other perspective-dependent information~\cite{SternbergVisualPerc}.
We will collectively refer to this set of high-level cues as contextual cues or more broadly as \emph{context}.

The full dependence on contextual cues of monocular depth estimation methods come with substantial challenges.
First of all, with the lack of any metric measurement of scene structure, monocular depth estimates are typically only able to reason the \emph{relative} depth of regions in the image as opposed to absolute depths that can be estimated with multiple calibrated cameras. 
As a result, monocular depth maps can only be used to reason about which object is closer to the camera and which one is further while the numerical depth difference between objects are left ambiguous.
The main challenge for monocular depth estimation, however, comes from the full dependence on high-level cues. 
Networks trained for depth estimation must represent semantics, texture properties, perspective cues such as vanishing lines, and an expected overall structure of the scene such as a horizon in outdoors scenes at the same time.
The performance of monocular depth estimation networks, as a result, heavily depends on the amount and the spatial distribution of these contextual cues in the image.

Figure~\ref{fig:introcontext} shows the results of a state-of-the-art monocular depth estimation network Midas~\cite{midas} with changing context. 
As one can intuitively conclude, if the image has too few contextual cues, monocular depth estimation networks are not able to generate a reliable result. 
Too much context, on the other hand, results in blurry depth estimates in large parts of the image. 
This comes from the inherently limited capacity of neural networks~\cite{baldi2019capacity}.
These observations point to the fact that using input images with \emph{right amount of} context will result in better depth estimates.

%\putfigure{introcontext}

The resolution of the input image also have a substantial effect on monocular depth estimation results, as Figure~\ref{fig:introresolution} demonstrates. 
Inputs with higher resolutions typically result in sharper depth estimates. 
While some of this come from the fact that there is simply more information in larger images, we observed that even upscaling small input images results in sharper estimates. 
This points to the fact that the spatial distribution of contextual cues in the image has an important role in the ability of the network in making the best use of context. 
When the input image is very large, however, the distribution of contextual cues in the image gets too sparse. 
As a result, we also see a degradation of the depth estimates as the input image size gets larger and larger.

%\putfigure{introresolution}

In this paper, we use this dependency of monocular depth estimation networks on context in our favor to generate high-resolution sharp depth estimates. 
We present an analysis of context dependency using three state-of-the-art methods, Midas~\cite{midas}, MegaDepth~\cite{megadepth}, and SGR~\cite{sgr} in Section~\ref{sec:monoculardepth}. 
Using this analysis, we introduce a method that can generate high-quality monocular depth estimations by combining the results of a base network with changing context in Section~\ref{sec:method}. \yagiz{this part needs much better phrasing} Our proposed method is summarized in Figure~\ref{fig:pipeline}. Our contributions can be listed as:
\begin{itemize}
\negvspace\item Analysis of context dependency in monocular depth estimation networks,
\negvspace\item A method to merge two different monocular depth estimations into one,
\negvspace\item A method to generate high-quality estimations without limitations coming from too small or too large input resolutions,
\negvspace\item A method to estimate the right amount of context by adaptively selecting cropped regions in the image,
\negvspace\item And a pipeline to generate high-resolution depth estimations using pre-trained monocular depth estimation networks.
\end{itemize}




==> tex/method.tex <==
% !TEX root = ../depth.tex


We propose a method that adaptively increases the depth estimation resolution in different regions in the image depending on their context density by using a pre-trained monocular depth estimation network. 
Our approach is adaptive to the choice of the monocular depth estimation model and we report numerical results in Section~\ref{sec:results} using two different networks. 
We present our analysis in this section on MiDaS~\cite{midas}. The demonstrations in this section are presented for the structure-guided method by Xian et al.~\cite{xian2020sgr} in the supplementary material.

We start by generating a depth estimate for the whole image in Section~\ref{sec:wholeimage}, where we fuse high- and low-resolution estimates into one coherent estimation with fine-grain details in a scheme we call \emph{double estimation}. 
This approach makes the best use of the underlying network for whole-image estimation and we show in Section~\ref{sec:results} that it alone outperforms baseline approaches.
We then describe our patch selection method that adapts the patch size locally with respect to the context density in Section~\ref{sec:cropselection}.
We generate depth estimates for these patches and merge them onto our whole-image estimate using the merging network in Section~\ref{sec:merging}. 
We make use of this merging network also in our double-estimation scheme.
An overview of our pipeline is presented in Figure~\ref{fig:pipeline}.


\input{imagetex/merging}

\subsection{Whole-Image Depth Estimation}
\label{sec:wholeimage}

We showed in Section~\ref{sec:monocular} and Figure~\ref{fig:resolution} that low- and high-resolution depth estimates provide complementing advantages. 
Our analysis also showed that the low-frequency artifacts in high-resolution estimates originate from local low context density.
We start by formulating a way to determine the maximum resolution that keeps the maximum distance between the contextual cues lower than the receptive field size of the network. 
For this purpose, we need an estimation of the contextual cues present in the image. 
Hu et al.~\cite{hu2019visualization} propose a network to estimate the contextual cues in an image and use it in their analysis. 
However, their method failed to give us high-resolution estimations that we require. 
Following Hu et al.~\cite{hu2019visualization}'s observation about the strong correlation between image edges and contextual cues, we use an approximate edge map of the image obtained by thresholding the RGB gradients as a proxy for contextual cues.

We determine the resolution at which the contextual cues in the image are at most receptive field size apart by  applying binary dilation to the edge map. 
By making sure that each pixel receives edge information during the forward pass, we  avoid the low-frequency artifacts while maximizing the accuracy of the estimates. 
However, as detailed in Section~\ref{sec:merging}, we can use our merging network to fuse together a low- and high-frequency estimates to retain the overall structure in the scene while keeping the fine-grain details. 
Hence, we use a double-estimation scheme where we use the network output at the training size as the low-resolution estimate and generate our high-resolution estimate at the resolution where we allow 20\% of the pixels to be far away from contextual cues in the image. 
Figure~\ref{fig:doubleest} demonstrates that we successfully generate a stable high-resolution estimate beyond the maximum resolution allowed by the network. 
We present our quantitative analysis on double estimation in Table~\ref{tab:doubleest} and Section~\ref{sec:results:double}.

The resolution of our estimation does not depend on the original resolution but on the distribution of edges in the image. 
We demonstrated in Figure~\ref{fig:upsampledEst} that monocular depth estimation networks are able to generate more accurate results even if the input images are upsampled. 
However, we do not upsample to more than 3 times the original size because we empirically observed no performance gain beyond that limit. 

\subsection{Context-Dependent Patch Selection}
\label{sec:cropselection}

%Following our observation that regions with different context densities should be fed to the network at different resolutions, we select patches with different sizes across the image that has enough context in them. 
%We found that one critical criterion to get reliable depth estimates from patches is to make sure the availability of enough contextual cues. As we use the edge map in the image as proxy for contextual cues and that the fact that not all edges will provide useful information for depth estimation, we remain cautious in determining the minimum patch size in the image. 

We found that one critical criterion to get reliable depth estimates from patches is to assure the availability of enough contextual cues. To establish an estimation of the context density in the image, we use the edge map in the image as proxy for contextual cues. Specifically, we compute the edge map at the whole-image estimation resolution, providing a \emph{context map} $M$ which we leverage to determine robust patch sizes. %These influence regions will be used extensively to help us define robust patch sizes.

We start the patch selection procedure by defining a regular grid with a stride equal to the network's receptive field size and with an empirically determined 33\% overlap between neighboring patches.
For each patch, we search for the the optimal crop size starting at the network's receptive field size. For each candidate patch $P_i$, we measure its context percentage value $\mathcal{C}_{P_i}$:

\begin{equation}
\mathcal{C}_{P_i} = \frac{\sum_{p \in P_i}M(p)}{|P_i|}
\end{equation}

where $|P_i|$ denotes the area of the patch $P_i$. If this value is smaller than the context percentage of the whole image, $\mathcal{C}_{\text{whole}}$, we discard that patch for not having enough local contextual cues. If it is higher than $\mathcal{C}_{\text{whole}}$, we gradually increase the patch size until its context percentage hits this limit. This crop selection scheme is in the cautious side to make sure that each patch we use can generate stable high-resolution estimates.
%Figure~\ref{fig:cropoverview} shows an example patch selection process.

We generate the depth estimate for each patch using our double-estimation scheme to maximize the resolution while minimizing artifacts. We use our merging network (Section~\ref{sec:merging}) to embed the high-resolution patch estimates onto the whole image estimate obtained in Section~\ref{sec:wholeimage}. We embed the patch estimates from the largest patch in the image and progressively refine our base estimate by merging patches with decreasing sizes. As the effective receptive field size is smaller than the theoretical value \cite{luo2016understanding}, the estimations close to image borders are less reliable than the rest. We therefore use a feathering mask to update our full-size estimate after the merging operation, which discards the borders of the patch estimate and ensures a smooth transition.

Recall that with our search  approach, the maximum distance between depth cues is at most the network's receptive field size. This results in really small resolutions for images with non-uniform depth cue density. Fixing the crop size at the receptive field can result in effectively selecting too few crops in such images. In order to detect such images and use smaller crops or equivalently enlarge the target resolution so that the effective crop size decreases, we do the following adjustment. We determine this target resolution $\mathcal{R}_{\text{target}}$ based on the whole-image estimation size $\mathcal{R}_{\text{whole}}$ and the influential context percentage value $\mathcal{K}_{\text{whole}}$:
 
\begin{equation*}
    \mathcal{R}_{\text{target}} = 
    \mathcal{R}_{\text{whole}} 
    \max(1,\frac{1}{2*\mathcal{K}_{\text{whole}}} 
    \left(\frac{\mathcal{R}_{\text{max}}}{2*\mathcal{R}_{\text{whole}}}\right)),
\end{equation*}
%
$\mathcal{K}_{\text{whole}}$ is computed with the same logic of $\mathcal{C}_{\text{whole}}$, but we additionally dilate the binary edges map $M$ with a box kernel with quarter the receptive field size. This dilated edge map defines a small \emph{influence region} around each edge and $\mathcal{K}_{\text{whole}}$ measure the percentage of the these regions. If $\mathcal{K}_{\text{whole}}$ is big enough, --- and enough is empirically set to 50\% --- we enlarge the target with a factor related to it's current resolution and $\mathcal{R}_{\text{max}}$ ratio. Here, $\mathcal{R}_{\text{max}}$ denotes the upper-bound resolution, which we empirically set to $3000\times3000$ following our observation that this was the maximum resolution picked as $\mathcal{R}_{\text{whole}}$ for a 36-megapixel, high-gradient outdoor image. The max operation is used to ensure the factor will not make the target resolution smaller. This target resolution makes sure that we can select small high-density areas within a overall low density image with small patches when we define the minimum patch size the same as the receptive field size in the selected resolution. 

%We assume that for a coverage of 50$\%$, $2*\mathcal{R}_{\text{whole}}$ is a sufficient base size \LM{Mahdi, Sebastian, please make this point clearer}. 



%For a lower coverage, $\mathcal{R}_{\text{base}}$ should be increased.  \yagiz{Mahdi, Sebastian, explain the mult. with 2's here} \SD{added explanation}.

%We start by defining a base size onto which the patch estimates will be embedded. 
%This base size is by definition larger than our whole-image estimate as the patches will be fed to the network at higher resolutions for a sharper result. 


%We generate the depth estimate for each patch using our double-estimation scheme to maximize the resolution while minimizing artifacts. 
%Since we have normalized $\mathcal{R}_{\text{base}}$ and $\mathcal{R}_{\text{whole}}$ and determined the size of the patches based on the local context density, we can select a fixed estimation resolution for patches.
%We set the low-resolution estimate to the receptive field size of the network and the high-resolution estimate to twice that size.
%This results in a direct correlation between the patch size and the effective resolution of the depth estimate in our final result, which is visualized in Figure~\ref{fig:cropoverview}.

%We use our merging network to embed the high-resolution patch estimates onto our base estimate. 
%This brings the range of values in the patch estimate to the range of values we expect for the whole image estimation. 
%We need to be careful to keep the full estimation consistent after merging. Since we know that the effective receptive field size is smaller than the theoretical value \cite{luo2016understanding}, the estimations close to image borders are less reliable than the rest. 
%We use a feathering mask to update our full-size estimate after the merging operation, which discards the borders of the patch estimate and ensures a smooth transition.

%We start embedding the patch estimates from the largest patch in the image and progressively refine our base estimate by merging patches with decreasing sizes.

\subsection{Merging monocular depth estimations}
\label{sec:merging}
In our problem formulation, we have a two depth estimations that we would like to merge together: (i) a low-resolution map obtained with a smaller-resolution input to the network such as a patch taken from our base estimate and (ii) a higher-resolution depth map of the same scene or patch that has much better accuracy around depth discontinuities but comes with a different range of depth values which may suffer from low-frequency artifacts coming from low local context density.
Our goal is to embed the high-frequency details of the second input into the first input which provides a general structure and depth range that is consistent for the full image. 

We adopt the pix2pix architecture~\cite{pix2pix} with a 10-layer U-net~\cite{unet} as the generator and the default PatchGan for the discriminator. 
Our selection of a 10-layer U-net instead of the default 6-layer version in the original pix2pix~\cite{pix2pix} is to increase the training and inference resolution to $1024\times1024$, as we will use the merging network for a wide range of input resolutions. 
We train the network to transfer the fine grained details from the high-resolution input to the low-resolution input. 
For this purpose, we generate input/output pairs by choosing patches from estimates for selected images from Middlebury2014 \cite{Scharstein2014HighResolutionSD} and Ibims-1 \cite{Koch18}. %Despite the fact that there is no fixed input resolution that can generate consistent higher resolution images, we tried different resolutions and%% 
While creating the low- and high-resolution inputs is not a problem, a consistent and high-resolution ground truth cannot be generated natively. Instead, we empirically pick 672*672 pixels as input resolution the network which maximizes the number of artifact-free estimations over both datasets. To ensure that the ground truth and higher resolution patch estimation have the same amount of fine-grained details, we apply a guided filter on the patch estimation using the ground truth estimation as guidance. These modified higher resolution ground truth patches serve as a proxy for a seamless merged version of low-res and high-res estimation.

Figures~\ref{fig:doubleest} and \ref{fig:merging} demonstrate the success of our merging network in transferring the high-frequency details while removing low-frequency artifacts or depth ordering mismatches in the high-frequency input.


















































\iffalse
Our findings from Section~\ref{sec:monocular} help us optimize the performance of existing depth estimation networks without changing the underlying architecture or retraining.
We demonstrated in our analysis in Section~\ref{sec:monocular} that both the resolution (or the context density) and the amount of context is of the input image has immense effects in the final depth quality. 
We observed that coarse-scale estimation with the full image tend to preserve global structures, which while lacks fine-grained details can serve as the base to align local estimates.
This property can be exploited to fuse the complementary information from local and global estimate made by the same model into a highly detailed yet globally consistent overall depth map.
Hence, our main goal is to maximize the estimation quality of pre-trained monocular depth estimation networks by carefully choosing appropriate inputs that allow the network to flourish. 
We formulate a method that can adapt the network input to the changing local context density in the image by determining patches in the image with adequate context and optimizing their resolution before feeding them to the network. 
We then merge the depth from different patches into one coherent depth map for the whole image.

The observations above provide the basis of our patching-aware framework. Figure \ref{fig:pipeline} illustrates our overall method. 
Given an input image, we first apply the full-image depth estimation and upsample the resulting depth map to the target image resolution to obtain the base estimate.
Note that we could use the training-resolution in generating this base estimate. 
However, we adaptively identify the appropriate resolution with which a more accurate whole-image depth estimate can be achieved with a double-estimation scheme as discussed in Section~\ref{sec:wholeimage}.
We then analyze each local image region and identify the appropriate patches with enough contextual cues and feed the patch into the depth estimation model, resulting in the corresponding context-adaptive local estimate in Section~\ref{sec:cropselection}.
The patching module detailed in Section~\ref{sec:merging} is then used to combine individual local estimations with the base estimate to generate the high-resolution result.

%We start by generating a depth estimation for the whole image.
%This whole image estimation will serve as the base to which we merge the patch estimations.
%In Section~\ref{sec:wholeimage}, we describe how we go beyond the quality of maximum stable resolution that the whole image can be fed to the network by combining whole image estimations obtained at two different resolutions. 
%This base depth map provides an anchor for the distribution of estimated depth values.
%We then select patches from the image with adaptive sizes depending on the context density of different regions in the image and generate high-resolution depth estimations in Section~\ref{sec:cropselection}.
%We progressively merge these patches into the base depth map to generate our final result.
%We will depend on merging for both base estimation and patch-based estimations, so we start our discussion with our methodology for merging different monocular depth estimates with the unique challenges it presents in Section~\ref{sec:merging}.

When determining the appropriate resolution for the whole-image estimation and selecting appropriate patches, we need an understanding of the distribution of the contextual depth cues in the image. 
Hu~et~al.~\cite{hu2019visualization} proposes a training scheme to estimate the contextual cues given a pre-trained network and use it in their analysis of important depth cues in different scene structures such as indoors and outdoors images. 
This approach failed to give us a high-resolution estimation of available depth cues for varying scene structures which we depend on when selecting local patches with enough context. 
Instead, we use an edge map we generate with a simple thresholding on the RGB gradient magnitude \yagiz{as shown in a figure maybe?}.
Hu~et~al.~\cite{hu2019visualization} specifically notes the strong correlation between contextual cues and image gradients, and our experiments also show that it is an adequate estimate of context that can be generated at high resolutions with ease.

\putfigure{merging}

\subsection{Merging monocular depth estimations}
\label{sec:merging}

Depth estimation results generated locally at different local regions, while giving accurate local details, are often not consistent with each other globally. Simply pasting local depth estimation into the high-resolution canvas results in a highly inconsistent overall depth map as illustrated in Figure~\ref{fig:merging}. 
This is coming from the fact that monocular depth estimation networks can only generate \emph{relative} depth ordering between regions in the image rather than a true depth map and the range of values in the generated result are fixed at $[0,1]$ regardless of the true range of depths in the scene.
As a result, the depth range from whole-image estimation inside a patch is smaller than the depth range of depth estimation from that patch.
Moreover, monocular depth estimates do not preserve the relative depth differences between image regions, only the ordering is preserved. 
As a result, we can not determine a simple global mapping function of depth values from the patch estimates to our base estimate.

In our problem formulation, we have a two depth estimations that we would like to merge together: (i) a low-resolution map obtained with a smaller-resolution input to the network such as a patch taken from our base estimate and (ii) a higher-resolution depth map of the same scene or patch that has much better accuracy around depth discontinuities but comes with a different range of depth values and may suffer from low-frequency artifacts coming from low local context density.
Our goal is to embed the high-frequency details of the second input into the first input which provides a general structure and depth range that is consistent for the full image. 

We adopt the pix2pix architecture~\cite{pix2pix} with a 10-layer U-net~\cite{unet} as the generator and the default PatchGan for the discriminator. 
Our selection of a 10-layer U-net instead of the default 6-layer version in vanilla pix2pix~\cite{pix2pix} is to increase the training and inference resolution to $1024\times1024$ as we will use the merging network for a wide range of input resolutions in Sections~\ref{sec:wholeimage} and \ref{sec:cropselection}. 
Instead of defining the task as a direct image-to-image translation task, we train the network to produce one-degree polynomials per-pixel. 
Estimation of this intermediate representation of the mapping instead of the final result allows us to train the network with more ease to avoid the typical GAN-artifacts which were present in the network trained for direct estimation. 

Our aim with the merging network is to embed high-frequency details onto our base estimate.
Most datasets with ground-truth depth, however, are of low-resolution with localization and discretization artifacts \yagiz{cite something here? maybe midas if they talk about this?} which does not allow training the network for high-resolution merging results. 
\yagiz{How we generate the training dataset and stuff here...}

We demonstrate the results our merging network generates in Figure~\ref{fig:merging} as well as in Figures~\ref{} in the following sections.

\putfigure{doubleest}

\subsection{Whole-image depth estimation}
\label{sec:wholeimage}

The first step of our method is generating a base estimation for the whole image that will define the target depth range and overall scene structure into which we will merge our patch estimations. 
We showed in Section~\ref{sec:monocular} that increasing the resolution at which we feed the whole image to the network increases the sharpness and the edge localization of the networks. 
However, when we increase the resolution too much, we also showed that the network starts generating low-frequency artifacts in the image when the depth cues in the image become further apart than the receptive field size of the network. 

We use an edge map of the RGB image as a proxy to contextual cues~\cite{hu2019visualization} and we can determine the point at which the context density hits it limit for a stable depth estimation.
We determine this resolution by dilating the edge map with a box kernel that is the same size as the receptive field size and making sure that every pixel in the image has closeby edges as shown in Figure~\ref{fig:doubleest}.
Notice that this resolution depends on the image content, more specifically the distribution of edges in the image, and it is in fact independent of the original resolution of the image.
This leads to one interesting observation about the monocular depth estimation networks: They are able to generate sharper depth estimates than their input image. 

Our merging network is trained to merge low-resolution estimations with a large resolution version of the depth estimate with higher resolution. 
One additional benefit of merging is that it can tolerate some low frequency artifacts in the high-resolution estimate that comes from too sparse contextual cues in the image. 
We use this power of our merging network to generate stable whole-image depth estimations that are of higher resolution and sharpness than the maximum resolution determined by the distance between image edges. 
We accomplish this by selecting an input resolution that leaves a portion of the image without any contextual cues in their vicinity, which generates sharper results with some low-frequency artifacts.
We then merge this estimation with a depth estimate we obtain by feeding the input image at the training resolution of the network, which provides stable overall structure for the scene.
Table~\ref{tab:doubleest} and Figure~\ref{fig:doubleest} show that we are able to generate sharper results with higher performance with this double estimation scheme when we allow 10\% of the pixels not to have nearby contextual cues. 
Making the context even more sparse exceeds the capacity of our merging network to remove the artifacts in the high-resolution estimate.

\subsection{Context-Aware Patch Selection}
\label{sec:cropselection}

%\input{imagetex/cropoverview}

- Find the optimal size for whole image est. This is equivalent to normalizing the image size with respect to minimum context density, which gives us a starting point to determine plausible patch sizes.

- We want smaller patches in dense context areas. Context map: dilated edge map with half receptive size.

- 

%\input{images/doubleest}
--\SD{current crop selection procedure:}
\begin{itemize}
    \item our assumption is that given an optimal size for the full image estimation, an optimal crop size for that image would be exactly the receptive field size. Since the upper bound within the double estimation for every crop is 2* receptive field size, the resolution of each crop can maximally be doubled. We an thus define the maximum resolution of the resulting depth map as 2*optimal size for full image estimation.
    \item we rescale the rgb image to that maximum resolution. we thereby also take the original resolution into account and define that no image shall be upscaled more than by a factor of 3 from its original size.
    Note that we keep the original aspect ratio while resizing (largest side gets set to maximum). Since we rescale the input image, the initial crop size can be fixed.
    \item we notice that the optimal size for full estimation can be misleading for crops: If an image has a high amount of gradients condensed at only a small part of the image, the optimal size will be relatively small. This will lead to crops which are too big for existing high gradient areas. In this special case, the gradient density is relatively low while the average gradient amount is relatively high. 
    \item to account for this, we introduce another scalefactor.
    \SD{todo: add description on scale factor, average gradient amount and gradient density}
    \item we take the edge map in optimal size and apply a dilation with 0.25*receptive field size(to dilate gradients reasonably) and calculate the percentage of ones in the dilated edge map($grad_p$).  scale factor is calculated as below:
    \[
    scalefactor = min((2grad_p)*(2\frac{optsize_{whole}}{optsize_{max}}),1)
    \]
    $optsize_{whole}$ is the global-adaptive optimal size calculated by us, $optsize_{max}$ is the maximum size $optsize$ can be(it is set to 3000 because in all our tests over all datasets and HD images the maximum size picked by global-adaptive search was $\sim2800$). min operation is to ensure that the scale factor won't result in crops bigger that receptive field. 
    
    \item we apply a grid of crops over the image with twice the receptive field size as cell size and 0.375* cell size as stride (we empirically found this to be the best stride size)
    \item we take the gradient image, threshold it so that every pixel smaller the mean is set to 0 and get calculate the gradient percentage per image (grad pixel/resolution)
    \item for each crop/ grid cell we select the corresponding part of the thresholded gradient image. If that parts gradient percentage is lower than the full image, we discard that location.
    \item else, we increase the cell size iteratively and check if its still over the full images gradient percentage. We select the biggest crop area that is still over that limit.
    \item we set the resizing step size to 32/scalefactor pixels: our minimum step size is 32 pixels. if we have increased the image size to account for the gradient distribution, we also increase the step size accordingly.
\end{itemize}

%The general findings from section \ref{sec:monocular} help us to optimize performance from existing depth estimation networks without changing the underlying architecture or retraining. First, we consider a single image: An optimal depth map would have a resolution as high as the input with a respective level of details. Furthermore, we expect it to be accurate in the relative ordering of objects within the scene and to be smooth for even surfaces. In order to get the most accurate depth ordering, we provide the network with as much context as possible, which is maximum in the full image. We rescale the image to the perceptive field size of the given depth estimation network and use this as base for our estimation. The result is consistent in the ordering of depth and smooth for even surfaces, but is missing most fine details from the scene. 
%Based on the context density, we determine now the highest feasible input resolution: for every upscale step by half the receptive field size, we check if the image gradients are still within a meaningful distance from each other.    The resulting resolution is fed to the network again. This second estimate is sharper and contains almost all details from the scene. At the same time, it is less smooth and likely to contains more artifacts in even, non-textured surfaces.
%As shown in section \ref{sec:monocular}, iteratively increasing the input size of the neural network results in a gradual transition from most accurate ordinal relations to most sharpest edges. From this follows that selecting a midpoint resolution would create a less sharper result than the high-res version, while being not as smooth as the low-res version. Instead, we are merging both estimations to keep the advantages we already gained. The principle is shown in figure \ref{fig:doubleest}.   

%\subsection{Merging depth estimations}
%\label{sec:Merging}
%\putfigure{doubleest}
%\SD{ToDo:add network figure}
%Combining two different depth estimations is an ill-posed problem: Since a monocular depth estimation network is ambiguous up to a scale, its estimations are only valid relatively among pixels of the image and the absolute depth value assigned to each pixel can be different for another image from the same scene. This becomes also visible when we feed different input scales and resolutions to the network or running it on different crops which correspond to the same image: absolute depth estimation values do not match for the same object.
%Because the scene content is the same for both images, we treat the merging as an image translation task. By merging, we are translating the characteristics of one input to the domain of the other. In other words, our merging network takes a pair of estimations and transfers the high frequency information from one input into the second one's ordinal relation estimation. \SD{need better phrasing here}.
%We base our merging network on the Pix2Pix architecture \cite{pix2pix} with 10-layer-U-Net as the generator and a L1-loss for the generator.\mahdi{We are using 10-layer-Unet.We are using the default loss terms proposed by pix2pix paper patchGan for discriminator architecture}. We add guided filtering to reduce merging artifacts. In order to make sure that absolute values will match completely, we also added a degree one (linear) polynomial fitting. 
Since we know that the effective receptive field size is smaller than the theoretical value and approximately Gaussian \cite{luo2016understanding} \SD{show in analysis section}, we generate a  Gaussian mask and use alpha blending to blend the merged result over the low-frequency estimation.

\fi

%\paragraph{Double estimation}
%As we mentioned in section ? \mahdi{where we discuss observations over networks behaviour for feeding higher resolution input} Estimations for higher resolution inputs can suffer from low frequency inconsistencies. We exploit the Merging network to address this issue. Whenever we are doing an estimation for an input with resolution bigger than network training resolution; for every such RGB input, we do two estimations. First one with resizing the input RGB image to the network training size and other with a bigger size that we select \mahdi{ how we select should be discussed in network behaviour with respect to resolution}. In the next step we use the merging network to merge fine-grained details from the higher resolution estimation to the low resolution version. We refer to this procedure as \textbf{Doubleestimation}. In section \ref{sec:results} we will show that this procedure increases our methods robustness for using higher resolution estimations compared to single resolution estimation. \LM{increase the robustness compared to what baseline?} 

%\mahdi{I am putting this paragraph here because I wanted to just put it somewhere so I don't forget about it :D} \SD{correlates with first paragraph of this section}
%For calculating whole image resolution we are assuming that depth cues are correlated to rgb image gradient. This assumption is mostly correct but in some cases we noticed that we are selecting a resolution which high for the special image. And also in some cases we are selecting a resolution which is smaller than the optimal one. in order to create a robust estimation we are using the double estimation also for the whole image estimation. We need a base estimation that we completely can trust which will be the network receptive field resolution and a higher resolution that we are calculating based on gradient density in the image. since we know our Mapnetwork is robust when it comes to high resolution estimation inconsistency then we are sure that using the calculated resolution with the doubleestimation method will generate a consistent high resolution depth.
%The way we are calculating the resolution contains a threshold that sets the amount of allowed regions in the image that there is not depth cue in the their neighbouring. Considering the ideal situation that gradients are the depth cues (not correlated but the same thing) then we can use the resolution calculated by setting this threshold to zero as the smaller size of double estimation but we know this assumption is not correct and we can not be sure if the estimation in this resolution is completely consistent.

% \paragraph{Double estimation} Now that we have a network that is capable of merging fine-grained high resolution depth information to a low resolution base depth map, we can use it every time we do an estimation not on the original resolution of the network. We define double estimation as estimating two depth maps for any RGB input - one with the resolution equal to receptive field size of the given depth estimation network and the other one with a higher resolution. We then use our \textbf{MergingNetwork} to merge these two and obtain a high resolution and accurate depth estimation. 

%\subsection{Selecting the right context and resolution } 
%\label{sec:CropSelection}
%For most natural images, we can assume that depth cues are not equally distributed across the whole image. Hence, we utilize our findings from section \ref{sec:monocular} once more to optimize depth prediction for individual areas within the image.

%\paragraph{Brute Force approach}
%A naive solution is the following: First, apply a regular grid of crops with the optimal resolution on the full image and get the estimation for each crop. And second, combine the individual estimations to create an enhanced disparity map for the full image.
%This approach however comes with a catch: As well as some crops have in fact a higher depth cue density than the whole image, others also have a far lower density. For this reason, it is more likely for crops to not contain enough depth cues for a network to reliably estimate depth. The resulting estimation will either be completely blurred or contain lots of artifacts. Also, following our observations about the ordinal relations within the scene, the crops will likely look less consistent. \mahdi{Magnified Object depth estimation will produce less consistent estimation for flat surfaces.}


%\paragraph{Image-guided approach}
%Our goal is instead to optimize the estimation for a certain area within the image with respect to the depth cues present.\\ We approximate the level of depth cues by the amount of gradients in the RGB image \cite{}. First, we select a fine grid as a base to scan the individual image regions. We set the initial cell size to half the receptive field size of the network. Since this size is fixed, it results in different portions of the image depending on the original resolution.
%In section \ref{sec:merging} we already determined the maximum possible resolution for the resulting depth map. We take this as an additional factor for the initial cell size into account since  \\
%Next, we analyze the crops with respect to the number of high gradient values per area: We empirically set the threshold between low and high gradients to the mean gradient magnitude per image. If the number of pixels corresponding to a high gradient within a crop is very high compared to that threshold, the area likely contains many depth cues and we keep it. If the number is low, we increase the size of the area in steps of 32 pixels per side to find more depth cues. If some bigger area A centered at the original grid cell passes our threshold while still being completely within the image borders, we replace the original cell by that area. If no bigger area with enough cues can be found, we discard the cell.
%Formally, we say:
%\begin{equation}
% todo
%\end{equation}
%  \LM{Here we should also be more specific to avoid confusion. What is the size of the coarse grid? What was the original crop size? Is it an absolute number or defined adaptively wrt. the image size? By how much did we reduce the crop size at every step?}

%
 
  
%\paragraph{Depth Cue Maps}
%\SD{This part becomes relevant when we have the results from the visualization paper}
%Learned depth cues from an existing network are valuable information to find optimal crop location, size and resolution. Recently, Hu et al.\cite{hu2019visualization} introduced a network which is trained to create masks for given depth estimation networks which eliminate all irrelevant pixels for depth prediction. We use their approach on MiDas to create depth cue maps, replacing all gradient maps we use for our analysis. 
  


%\subsection{Our pipeline} 
%In summary, our method involves four distinctive steps:
%\begin{enumerate}
%    \item Generating a baseline by merging two different estimations for the full image to combine highest sharpness with best consistency,
%    \item Selecting crops based on depth cues within the image for higher resolution details in these areas (section \ref{sec:CropSelection}),
%    \item generating two different estimates per crop and finally
%    \item merging the crops with the base image to create the final output (section \ref{sec:Merging}).
%\end{enumerate}

%\LM{The sequence of steps above only describe what was done for a single crop. It's not clear how to string those single-crop results together to make the full pipeline that generate the high-res depth map from the original low-res one.}
%\LM{A diagram depicting the pipeline will be very helpful here.} \SD{Added placeholder after next paragraph. ToDO: add actual figure}






%We conduct our experiments based on MiDas. Due to the similarities in behaviour of depth estimation networks as described in \ref{sec:monocular}, it is possible to select other current CNN-based depth estimation network instead and apply our procedure. \LM{We can perform experiments with one or two more methods, then we can say here that our technique generalize well across different depth estimation methods.}

%MiDas has a receptive field size of 384. We select this to be the lower bound for our double estimation and determine the upper bound as described above. \LM{I think we may need to be more specific here in terms of the empirical procedure we used to determine that optimal resolution, and which criteria did we base on to judge the quality}. \SD{removed the part the comment was referring to}

%Next, we apply our image-guided search approach on the RGB image and create a list of suitable crops with optimal size with respect to the underlying image context. We sort the list and generate a double estimation for each crop. Then, starting with the largest crop size, we select the corresponding area from our base estimation and merge the double estimated crop with that area using PatchingNet. The base estimation is iteratively updated by inserting the resulting pixel values at the crop position, until every crop is inserted. Figure \ref{fig:pipeline} is showing the procedure.   



\iffalse
\subsection{Merge(most of it is obsolete)}
\label{sec:Merging}
As we mentioned above, the raw cropped estimations are not reliable in low frequent depth areas. Using local mapping will help to largely reduce these behaviours, but can't fully eliminate them. Additionally, using a confidence map while doing the merging could be helpful: If the network output is weighted based on how reliable the estimated value is, less reliable values will have less effect on the merged result. \LM{We need to specify what this confidence map represent, e.g. what does each pixel value in this map mean?}. Low frequencies can reliably be estimated based on the full image, even if it's scaled down too much to preserve details. Merging the cropped depth maps with the full estimation based on a confidence map can eliminate low frequency artifacts while reproducing high frequency details.

\paragraph{Masking the input}
Confidence maps can be generated within MiDas based in the saliency information, which has been introduced in previous stages. We can expect the activations of the network to be higher for areas with a lot of depth cues. So the saliency map from MiDas encodes information about which pixels are actually important to determine the depth value and are therefor more reliable for the final result.
         \\
Another type of confidence map we can generate is based on the performance of the local mapping network. Since local mapping will never be perfect for high frequency areas, the mapping error will be high. Thus, we can use the inverted mapping error to down weight low frequency areas, which are prone to depth estimation errors in crops.
        \\
To apply the confidence mask on the estimated crop, both types can be used as alpha mattes:
The pixel values $P_{out}$ for each crop can be determined by
\begin{equation}
    P_{out}=\alpha P_{crop} + (1-\alpha) P_{base}. 
\end{equation}
Here, $P_{crop}$ is the pixel value of the crop and $P_{base}$ the value for the corresponding part within the base depth. We apply a Gaussian blur on the confidence map $\alpha$ to encourage smoothness. Additionally, we found that adding a circular feathered mask $M$ to $\alpha$ greatly helps reducing visible borders between individual crops. \LM{It seems that we have two different ways for confidence map (saliency map and inverted error map), which one are we using as $\alpha$ here?}

  
\fi



==> tex/method_backup.tex <==
% !TEX root = ../depth.tex

\newcommand{\fgt}{$\mathcal{F}$}
\newcommand{\bgt}{$\mathcal{B}$}
\newcommand{\unt}{$\mathcal{U}$}
\newcommand{\knt}{$\mathcal{K}$}
\newcommand{\ggt}{$\mathcal{G}$}
\newcommand{\wholet}{$\mathcal{I}$}

\newcommand{\fgm}{\mathcal{F}}
\newcommand{\bgm}{\mathcal{B}}
\newcommand{\unm}{\mathcal{U}}
\newcommand{\knm}{\mathcal{K}}
\newcommand{\ggm}{\mathcal{G}}
\newcommand{\wholem}{\mathcal{I}}



\putfigure{pipeline}

\yagiz{Plan for the method part:}

Overview of method -- first do full-image estimation and then do cropped ests.

1 - Merging two estimations

2 - Choosing the right resolution

3 - Choosing the right context

4 - Full pipeline

The general findings from \ref{sec:monocular} help us to optimize performance from existing depth estimation networks without changing the underlying architecture or retraining. First, we consider a single image: An optimal depth map would have a resolution as high as the input with a respective level of details. Furthermore, we expect it to be accurate in the relative ordering of objects within the scene and to be smooth for even surfaces. In order to get the most accurate depth ordering, we provide the network with as many depth cues as possible, which are naturally given in the full image. We rescale the image to the perceptive field size of the given depth estimation network and use this as base for our estimation. The result is consistent in the ordering of depth and smooth for even surfaces, but is missing most fine details from the scene. 
We know that higher resolution depth cues result in higher depth map sharpness, so we upscale the image to twice the receptive field size next and feed it to the network again. This second estimate is sharper, but less smooth and likely to contain artifacts in even, non-textured surfaces. Instead of searching for an in between resolution, which would create a less sharper result than the high-res version, while being not as smooth as the low-res version, we are merging both estimations to keep the advantages we already gained. The principle is shown in figure \ref{fig:doubleest} We introduce a network based on Pix2Pix to merge the results, which will be explained in the next section.   

\subsubsection*{Merging network}
\label{sec:Merging}
\putfigure{doubleest}
 The merging network takes a pair of estimations and transfers the high frequency information from one of the input depth to other one's absolute value. We need a dataset containing two depth pairs as our network input; one with accurate low frequency depth value and one  with high resolution but not consistent low frequency and different depth value distribution. Additionally, it should contain a high resolution and low frequency consistent ground truth depth. To obtain such a dataset we exploit our observations at section ??? \mahdi{where we explained midasplus} and synthesised a dataset. We used pair of vanilla midas estimation on whole image as base estimation and cropped estimations as the high resolution but inconsistent as one of the pairs and midasplus estimations as the ground truth to train the network. In order to make sure that our cropped estimation and midasplus results have the equal amount of high frequency depth information; so that network will generate sharp results, we used guided filtering to blur the cropped estimations with the guidance of midasplus results. Since the formulation is close to image transfer techniques we adapted Pix2Pix\cite{pix2pix} architecture with 5-layer-Unet as the generator and trained for 200 epochs with L1 as the loss.
In order to make sure that absolute values will match completely we also added a degree four polynomial fitting. \mahdi{We may be able to relax the degree to one but needs more experiments on the final pipeline}
We can easily merge these smooth and high resolution patches to the base estimation by only replacing their values with corresponding pixel values in the base estimation.

\paragraph{Double estimation} Now that we have a network that is capable of merging high frequency depth information to a low frequency accurate depth map, we can use it for all our estimations. We define double estimation as estimating two depth maps for any rgb input - one with the receptive field size of the given depth estimation network and the other one with a higher resolution. We then use our \textbf{MergingNetwork} to merge these two and obtain a high resolution and accurate depth estimation. In section \ref{sec:results} we will show that this procedure increases our methods robustness compared to single scale estimation. \LM{increase the robustness compared to what baseline?} 

\subsection{Select Crop Location} 
        \label{sec:CropSelection}
Next, we look into further optimizing the depth prediction for individual areas within the image:
\SD{This part will most likely move to the analysis section}
As a first test, we randomly crop images such that each crop is exactly 672x672 pixels in resolution, and compare each crops estimation with the corresponding area in the full images' estimation from MiDas Plus.
\SD{ToDo: add test results for visual comparison}.
As it turns out, the crop-based estimation on average can distinguish more details in depth than the full image-based estimation, even when using MiDas Plus for the latter.

\paragraph{Brute Force approach}
This leads to the following brute-force approach: First, apply a regular grid of crops with the optimal resolution on the full image and get the estimation for each crop. And second, combine the individual estimations to create an enhanced disparity map for the full image.
This approach however comes with a catch: While we can assume that in most natural images enough depth cues are present to get a reasonable depth estimate, this assumption does not hold for every subarea in that image. For this reason, it is far more likely for crops to not contain enough depth cues for a network to reliably estimate depth. The resulting estimation will either be completely blurred or contain lots of artifacts. Also, following our observations about the ordinal relations within the scene, the crops will likely look less consistent. \mahdi{Magnified Object depth estimation will produce less consistent estimation for flat surfaces.}
\\
The Network was able to generate consistently good depth estimation if it was fed with reasonable crop ( a crop with reasonable amount of contextual information). \LM{It might be a good idea to show some visual examples here to illustrate what we meant by this.} \mahdi{TODO: generate some examples for over-magnifying}
\SD{changed position}

\paragraph{Image-guided approach}
Instead, our goal is to optimize the estimation for a certain area within the image with respect to the depth cues present.\\ We approximate the level of depth cues by the amount of gradients in the RGB image \cite{}. First, we select a fine grid as a base to scan the individual image regions. We can assume depth cues within small images to be more densely packed than in large images, so we set the size of one grid cell to be dependant on the image scale. A starting cell size of $1/3$ of the smaller dimension of the image with a stride of half that size gave the best results in our experiments.\\
Next, we analyze the crops with respect to the number of high gradient values per area: We empirically set the threshold between low and high gradients to the mean gradient magnitude per image. If the number of pixels corresponding to a high gradient within a crop is very high compared to that threshold, the area likely contains many depth cues and we keep it. If the number is low, we increase the size of the area in steps of 32 pixels per side to find more depth cues. If some bigger area A centered at the original grid cell passes our threshold while still being completely within the image borders, we replace the original cell by that area. If no bigger area with enough cues can be found, we discard the cell.
Formally, we say:
\begin{equation}
 todo
\end{equation}
  \LM{Here we should also be more specific to avoid confusion. What is the size of the coarse grid? What was the original crop size? Is it an absolute number or defined adaptively wrt. the image size? By how much did we reduce the crop size at every step?}
  
\iffalse
\paragraph{Semantically guided approach}
A more sophisticated solution is to use a segmentation network to detect individual objects in the image and do a multi-resolution crop and estimation for each target object to refine the baseline depth.
We test a state-of-the-art network \cite{aksoy2018semantic} for Semantic Separation to output semantic features and
cluster the features into individual, continuous areas.\SD{todo: explain clustering and number of areas}.
However, some images by nature are not semantically separable, so no straight definition of salient objects was able to be introduced. Furthermore, to our knowledge there exists no neural network yet which is reliably able to detect all object classes present in images in the wild. So the feature vectors could only be used in a very limited scenario. For these reasons, we decided to rely on the Image-guided approach for our pipeline.
\\
\fi



\iffalse
Since MiDas as a monocular depth estimation network is ambiguous up to a scale, its estimations are only valid relatively among pixels of the image and the absolute depth value assigned to each pixel can be different for another image from the same scene. This becomes problematic when running the network on different crops which all correspond to the same image: absolute depth estimation values from different magnified region do not match for the same object. In addition, the absolute values from cropped estimation doesn't match with the values of our base estimation. Also, as we mentioned in section???  \mahdi{wherever we explained network behaviour for using bigger input size} cropped estimations tend to have inconsistent low frequency behaviour. As a result we need to \textit{map} our cropped region estimation values to the absolute values of the base estimation to be able to merge them into base estimation. in order to have a more robust mapping with regard to our estimation characteristics and to map these estimations to match the absolute values of a base estimation we trained a network. \textit{MapNetwork}.
\fi


Our results are based on work from Ranftl et al. \cite{midas}, which we will refer to as MiDas. Due to the fundamentally similarities in behaviour of depth estimation networks as described in \ref{sec:monocular}, it is possible to select any current depth estimation network instead and apply our procedure. \LM{We can perform experiments with one or two more methods, then we can say here that our technique generalize well across different depth estimation methods.}
\SD{ToDo: Add results from MegaDepth. Add results from a second network}

\subsection{Estimate the full image} 
    \label{sec:FullEst}
The first step of our pipeline involves generating a first depth estimation from the whole image, which is going to be used as the baseline.\\
The original implementation of MiDas was trained with images of size 384x384. Based on the first intuition about the network capacity, it is logical to test different input sizes for the depth estimation network.\\
We augmented images from Ibims1\cite{Koch18} and TAU\cite{haim2018depth} dataset by random cropping and resized each image to $\{(384+32n)*(384+32n)| n=0,1,2,...,30\}$ sizes (multiple of 32 was because of MiDas decoder constraint) and fed them to the network and evaluate the results based on  DDR\cite{whdr}. As expected, increasing the input size for MiDas results in sharper details in the disparity map. But at the same time, the consistency between different parts of the images is reduced. We empirically found that there exists a "optimal" spatial resolution of 672x672 pixels at which disparity edges are relatively sharp and the whole map is still relatively consistent. However, we aim to get results with the best possible combination of both worlds. Instead of settling with a single estimation, we decide to estimate twice: one estimate with the original input size for highest consistency and one estimate with twice that input size for the sharpest result.  \LM{I think we may need to be more specific here in terms of the empirical procedure we used to determine that optimal resolution, and which criteria did we base on to judge the quality}.
\iffalse
We refer to the original MiDas setup as "vanilla MiDas" and to the modified one as "MiDas Plus". Note that using MiDas Plus on its own will already increase the depth estimation accuracy.\\
Interestingly, we found that upscaling lower resolution images to higher input sizes for MiDas also increases the depth estimation. This becomes useful when creating training data for fine-tuning and evaluation (see section \ref{sec:Training}). 
\fi









\subsection{Estimate depth}
\iffalse
\SD{not enough for own subsection }\\
Generally, depth estimation networks are prone to be biased towards input data. We noticed that simply horizontal-flipping the input image can cause changes in the networks result. we can leverage this behaviour to augment possible depth values for each pixel.
\SD{Worth a shot, but we haven't tried that yet}
\fi

\paragraph{Depth Cue Map}
\SD{This part becomes relevant when we have the results from the visualization paper}
Learned depth cues from an existing network are valuable information to both distinguish useful crops from bad ones and get confidence values for the resulting depth maps. We decided to output saliency maps for each crop as well as for the full image estimation to be used in the rest of the pipeline.
\\            
Saliency maps are a common way in classification tasks to visualize which parts of an image are creating the highest activations and therefor resulting in a specific class $c$ as output \cite{Simonyan2014DeepIC}. More specifically, an artificial image I is created such that it results in the highest class score $S_c$ with:
\begin{equation}
    \argmax_IS_c(I)-\lambda||I||^2_2.
\end{equation}
Since we are not interested in a specific class, $S_c$ in our case becomes $S$. \LM{Is there existing work that compute saliency map from depth prediction model in this way? This formulation seems a bit odd to me because the depth map value has very different physical meaning from the class probability value from classification networks.}
\SD{ToDo:Add backpropagation}            

        


\iffalse
\subsection{Merge(most of it is obsolete)}
\label{sec:Merging}
As we mentioned above, the raw cropped estimations are not reliable in low frequent depth areas. Using local mapping will help to largely reduce these behaviours, but can't fully eliminate them. Additionally, using a confidence map while doing the merging could be helpful: If the network output is weighted based on how reliable the estimated value is, less reliable values will have less effect on the merged result. \LM{We need to specify what this confidence map represent, e.g. what does each pixel value in this map mean?}. Low frequencies can reliably be estimated based on the full image, even if it's scaled down too much to preserve details. Merging the cropped depth maps with the full estimation based on a confidence map can eliminate low frequency artifacts while reproducing high frequency details.
\paragraph{Masking the input}
Confidence maps can be generated within MiDas based in the saliency information, which has been introduced in previous stages. We can expect the activations of the network to be higher for areas with a lot of depth cues. So the saliency map from MiDas encodes information about which pixels are actually important to determine the depth value and are therefor more reliable for the final result.
         \\
Another type of confidence map we can generate is based on the performance of the local mapping network. Since local mapping will never be perfect for high frequency areas, the mapping error will be high. Thus, we can use the inverted mapping error to down weight low frequency areas, which are prone to depth estimation errors in crops.
        \\
To apply the confidence mask on the estimated crop, both types can be used as alpha mattes:
The pixel values $P_{out}$ for each crop can be determined by
\begin{equation}
    P_{out}=\alpha P_{crop} + (1-\alpha) P_{base}. 
\end{equation}
Here, $P_{crop}$ is the pixel value of the crop and $P_{base}$ the value for the corresponding part within the base depth. We apply a Gaussian blur on the confidence map $\alpha$ to encourage smoothness. Additionally, we found that adding a circular feathered mask $M$ to $\alpha$ greatly helps reducing visible borders between individual crops. \LM{It seems that we have two different ways for confidence map (saliency map and inverted error map), which one are we using as $\alpha$ here?}
\paragraph{Merging}
We assume that local mapping in combination with the confidence map already bring the cropped estimation close to the full estimation. Hence, a naive merging can be done via simply averaging the depth values:
\begin{equation}
    P_{out}=\frac{1}{2}(P_{crop}+P_{base}).
\end{equation}
Note that the base gets updated for every crop, so it includes the merged results from all crops before.
The results are plausible and can display most of the details. However, this approach is more prone to copy low frequency artifacts into the final result, if they haven't been fully eliminated in a crop. \\
Alternatively, a rank-based approach can be used to merge crops and base depth. Since every pixel is present in multiple crops (multi-resolution cropping or overlaying crops), we rank the individual depth values per pixel based on their occurrence. If the depth values in different crops are spread over a wide range of values, this indicates that the value is not reliable and we take more from the full estimation into account. If every crops has the same value for that pixel, the value should be very reliable and gets a higher rank associated.
More specifically, for a pixel $P$ with values $P={p_1,p_2,...p_n}$ we calculate the new pixel value $P_out$ by
\begin{equation*}
    P_{out}=mode(P).
\end{equation*}
Lastly, the highest rank wins and the pixel value is set accordingly.
With this, the low frequency artifacts can be fully eliminated. However, it isn't able to reproduce as many details as average merging.
Since the local mapping network and the confidence maps in combination are already eliminating all artifacts in our tests, we're selecting average merging in our experiments.   
\fi

In summary, our method involves four distinctive steps:
\begin{enumerate}
    \item Generating a baseline by merging two different estimations for the full image to combine highest sharpness with best consistency (section \ref{sec:FullEst}),
    \item Selecting crops based on depth cues within the image for higher resolution details in these areas (section \ref{sec:CropSelection}),
    \item generating two different estimates per crop(section \ref{sec:Mapping}) and finally
    \item merging the crops with the base image to create the final output (section \ref{sec:Merging}).
\end{enumerate}

\LM{The sequence of steps above only describe what was done for a single crop. It's not clear how to string those single-crop results together to make the full pipeline that generate the high-res depth map from the original low-res one.}

\LM{A diagram depicting the pipeline will be very helpful here.}

==> tex/monocular_long.tex <==

%As our main goal is to adapt existing models to higher resolution without re-training, we start by studying how different resolution-related factors in the input content affect depth estimation performance. Toward this goal, we study the depth estimation performance of different depth estimation models both at the image level and region level while systematically varying the input resolution and amount of information present in the input. 

Toward the goal of adapting depth estimation models to higher resolution, we investigate how the depth estimation performance changes with respect to the input resolution as well as its enclosed context. We look into depth estimation results generated from state-of-the-art depth estimation models with varying the input resolution and amount of information present in the input. We present our observations in this section with the results from MIDAS~\cite{midas} which is one of the most widely used method recently. We also observed similar results from two other models ~\cite{li2018megadepth} and \cite{xian2020sgr}, which are detailed in our supplementary materials.

\textbf{Local depth estimation quality is context-dependent} 
%The central idea of our method is that high-resolution images are composed of smaller local regions with well-defined content. 

It has been suggested in recent works that the predicted depth quality depends on the amount of contextual information present in the input image, in particular how the visual elements are arranged and distributed in relation with each other. Importantly, we observe that this context-dependence property apply not only when performing depth estimation the image level but also at each local image region. For further investigation, we randomly select ?? local regions from ?? images from the ?? dataset. For each local region, we generate ?? crops with sizes ??, ??, ..., ?? centered at the selected region. We feed all resulting cropped images to MIDAS and measure the performance by comparing to the ground-truth depth map at the corresponding local regions. Figure \ref{fig:analysis_local_context} shows that different local image region have different optimal crop size and resolution. This suggests that local depth prediction for each region can be optimized by determining the appropriate cropping windows. 

\textbf{Depth estimation results from different input resolutions give complementing advantages} 

While most depth estimation methods follow the common practice of training with a pre-defined and relatively low input resolution, the models architecture themselves are fully-convolutional which in principle can handle arbitrary input sizes. A natural question arises: does the model always produce the most accurate depth map at the training resolution for every images? To explore this question, we collect ?? Images from the ?? datasets with resolution ?? Which are beyond the typical training resolution of depth estimation models. For each of these images, we generate ?? different versions of the input by resizing the original image into ?? Different resolutions ??, ??, ??, ... ??. We feed each version of the input into a pre-trained depth estimation network, and upscale the result back to the original resolution using bilinear up-sampling before comparing with the ground-truth depth map. Figure \ref{fig:analysis_resolution} shows the depth map accuracy with the same inputs at different resolution. This result indicates that the optimal input resolution varies with different images, and the optimal resolution is often not the training resolution. \LM{In explaining why this is the case, we can provide more details regarding the relation between resolution and context density, including discussion on receptive field size}  

Looking into the depth estimation results from different input resolutions, we found that there is often no result that is superior than the others in all aspects. Importantly, we observe complementary advantages in depth maps generated from different input resolution. Low-resolution estimation tend to preserve global structures and consistency while lacking fine-grained details. As the input resolution increase, the depth estimation results exhibits increasingly sharper details but often suffer from inconsistent depth values, especially in large uniform regions (Figure~\ref{fig:resolution}). Fusing depth estimation results generated at different resolution can potentially make the best of both worlds and improve over each individual result. 

\yagiz{merging discussion moved to the method part}
%\textbf{The challenge of combining local depth estimation} \LM{We can consider moving this to the method section where we discuss the patching procedure}

%Depth estimation results generated locally at different local regions, while giving accurate local details, are often not consistent with each other globally. Simply pasting local depth estimation into the high-resolution canvas results in highly inconsistent overall depth map as illustrated in Figure~\ref{fig:global_local_complementary}. On the other hand, coarse-scale estimation with the full image tend to preserve global structures, which while lacks fine-grained details can serve as the base to align local estimates. This property can be exploited to fuse the complementary information from local and global estimate made by the same model into a highly detailed yet globally consistent overall depth map.

%\noindent\textbf{Depth estimation performance varies with different resolutions} 

%While most depth estimation methods follow the common practice of training with a pre-defined and relatively low input resolution, the model architectures themselves are fully-convolutional which in principle can handle arbitrary input sizes. A natural question arises: does the model always produce the most accurate depth map at the training resolution for every images? To explore this question, we collect ?? images from the ?? datasets with resolution ?? which is beyond the typical training resolution of depth estimation models. For each of these images, we generate ?? different versions of the input by resizing the original image into ?? different resolutions ??, ??, ??, ... ??. We feed each version of the input into a pre-trained depth estimation network, and upscale the result back to the original resolution using bilinear up-sampling before comparing with the ground-truth depth map. Figure \ref{fig:analysis_resolution} shows the ... \LM{Todo: elaborate the results}. 

%This result indicates two important points: 1) The best depth estimation result are often obtained neither at the training low resolution nor the very high resolution, and 2) Different images tend to have different optimal resolutions.  

%This result indicates that for a given image content, there often exists an input resolution other than the training resolution that give better performance. Furthermore, we found that the optimal resolution for a given image depends on how different information is distributed over the image space. \LM{Todo: elaborate on the context density here} 

%\noindent\textbf{Local depth estimation quality is context-dependent} 

%The analysis above and the findings from previous works \cite{hu2019visualization, howdepthestwork} indicate that the predicted depth quality depends on the content in the inputs image, in particular how the visual elements are arranged and distributed in relation with each other. Importantly, we found this context-dependence property apply not only when performing depth estimation at the image level but also when applying the depth estimation model at local image regions. For further investigation, we randomly select ?? local regions from ?? images from the ?? dataset. For each local region, we generate ?? crops with sizes ??, ??, ..., ?? centered at the selected region. We feed all resulting cropped images to MIDAS and measure the performance by comparing to the ground-truth depth map at the corresponding local regions. Figure \ref{fig:analysis_local_context} shows that different local image regions have different optimal crop sizes. This suggests that local depth prediction for each region can be optimized by determining the appropriate cropping windows.  

%\noindent\textbf{Global and local depth estimation are complementary}

%Depth estimation results made for the same content but at different resolutions tend to complement one another. Coarse-scale estimation tend to preserve global structures and consistency while lacking fine-grained details. On the other hand, depth estimation results generated locally at different local regions, while giving accurate local details, are often not consistent with each other globally. Simply pasting local depth estimation into the high-resolution canvas results in highly inconsistent overall depth map as illustrated in Figure~\ref{fig:global_local_complementary}. This property can be exploited to fuse the complementary information from local and global estimate made by the same model into a highly detailed yet globally consistent overall depth map. \LM{Todo: re-arrange the sentences to make the flow smoother}

\yagiz{the method overview here moved to the method section}
%The observations above provide the basis of our patching-aware framework. Figure \ref{fig:pipeline} illustrates our overall method. Given an input image we first apply the full-image depth estimation and up sample the resulting depth map to the target image resolution to obtain the base estimate. Note that we could use the training-resolution in generating this base estimate. However, motivated by observation 1, we adaptively identify the appropriate resolution with which a more accurate full-image depth estimate can be achieved. We then analyze each local image region and identify the appropriate cropping windows and feed the cropped region into the depth estimation model, resulting in the corresponding context-adaptive local estimate. The patching module is then used to combine individual local estimate with the base estimate to obtain the final depth estimation result. 

==> tex/related_orig.tex <==
% !TEX root = ../depth.tex

\paragraph{Single Image Depth Estimation}
Zhu et. al. \cite{zhu2020edge} use the boundary information from a semantic separation network to finetune a depth estimation network during training.
\SD{We should test against this.}
Hu et. al.\cite{hu2019revisiting} extend an encoder-decoder network by a feature fusion block. Together with a triple loss for depth, gradients and surface normals, this architecture aims for more accurate depth prediction around object edges.

A similar strategy is followed by Ranftl. et. al. \cite{midas}. Instead of applying a loss directly on predicted depth values, they design a scale-and-shift invariant loss in combination with a gradient-matching term to make the network robust against different data distributions during training.

Zhang et al. \cite{zhang2019pattern} propose to utilize pattern affinities between semantic segmentation, normal prediction and depth estimation and to combine them into a joint training method.   

Godard et al. \cite{godard2017unsupervised} utilize stereo footage as replacement for less available ground truth depth data. Given such an image pair, their method estimates the disparity which combined with one of the images can be used to reconstruct the other.

In a follow-up paper, Godard et al. \cite{monodepth2} refine their method by implementing a new reprojection loss to handle occlusions and a multi-scale sampling strategy to upscale estimation from intermediate network layers.

Lee et al. \cite{lee2019monocular} use a network with a multi-scale decoder, which estimates up to 10 relative depth maps with the ordinal relations for an image at different resolutions. Together with a regular depth estimation as baseline, the relative depth maps are decomposed into multiple depth components, representing details at different scales. These components are then combined to generate both an accurate depth distribution as well as a high level of details. 


Li et al. \cite{li2017two} use a two-stream network to estimate dense depth values and depth gradients from a single RGB image, which are then combined to create detailed depth map.


Sun et al. \cite{sun2020single} train a single image depth estimation network by using stereo pairs as ground truth.

Wang et al. \cite{wang2020cliffnet} suggest to apply a loss in a Hierarchical Embedding Space which is learned by a neural network, rather than comparing depth estimation output and ground truth directly on a pixel level. They further refine their approach using a hierarchical feature fusion network during upsampling.

Tang et al. \cite{tang2019neural} have introduced a neural network specialized on depth estimation for human figures. They split the task into two different streams by estimating a smooth base shape and high level details separately.

Fang et al. \cite{fang2020towards} analyze different aspects of common depth estimation networks like architecture, loss functions, data size and resolution with respect to their influence on the resulting estimations. Based on their findings, they introduce an optimized architecture. \SD{Needs more details, also maybe better in the analysis/network behavior part} 

Yin et al. \cite{yin2019enforcing} add 3D geometric constraints to depth estimation. In addition to regular depth supervision based on ground truth depth maps, they reconstruct 3D point clouds from their depth estimations and evaluate them against ground truth point clouds based on surface normals during training.

Huynh et al. \cite{huynh2020guiding} include a depth attention module within an encoder-decoder network structure. The main assumption is that depth values for two points on the same planar surfaces are linearly dependent. Given the first point, the second point is therefore easier to determine. The attention module is learning to construct a depth attention volume from ground truth data, which incorporates these linear dependencies for an image and increases the accuracy for texture-less areas.  

Zheng et al. \cite{zheng2018t2net} address the problem of little available training data for monocular depth estimation by introducing a two-stage strategy. They combine generated synthetic rgb/d image pairs with unpaired real images and use a GAN in the first stage to translate the synthetic images into real-world domain with the real images as target. The converted images then serve as training data for a depth estimation network.

Chen et al. \cite{depthattentionmodel} used "spatial attention module to create a structure-aware neural network. These basic blocks guided neural network attention to global structures or local details". \mahdi{They also gathered a hard-case depth dataset that might be used for evaluation}  

Lee et al. \cite{lossrebalancing} are proposing a method to combine multiple loss terms that adaptively changes the weights between different losses and makes sure that non of them is neglected during training.

\paragraph{Depth Refinement/Reconstruction}
Luo et. al. \cite{luo2020consistent} use disparity information from different video frames to finetune a pretrained depth estimation model ( one tested version is MiDas) to create temporal consistent depth. Since we're targeting single image depth prediction, this is not applicable in our case. \SD{Not sure if we should include video depth frameworks at all. But this paper got a lot of attention recently. Maybe a nice method to showcase our results?}

Heo et al. \cite{wsmrefinement} proposed a novel filter to exploit tendancy that a scence has similar depth in horizontal or vertical directions. They proposed a CNN that combine the mentioned filter with a Resnet decoder. They also estimate the reliablily of the esimated depth and use that in a CRF to refine the estimated depthmap. 

Eldesokey et al. \cite{uncertaintydepthcompletion} propose an approach to detect the disturbed depth input and propose a probabilistic version of NCNN that produces meaningful uncertainty measures. Their model only containing 670k models performs on-par with conventional approaches with millions of parameters.

\textbf{Feature Upsampling}
Recently, Zuo et. al. \cite{zuo2020frequency} proposed a upsampling-based approach in combination with a residual training, where low-level depth features are upsampled during inference to generate higher detailed results and filter out artifacts.
Durasov et al. \cite{durasov2019double} introduce also an approach based on feature upsampling. However, They mainly focus on efficiency and target mobile devices.

Zhao et. al. \cite{zhao2017single} handle blurry object boundaries by upsampling the estimated depth map. They use a residual dictionary learning approach to estimate the residuals for every upsampling step and apply an edge-guided weighted median filter to decrease noise and artifacts.

Wang et al. \cite{semanticconquerdepth} porpose a model that decomposes the scence into semantic segments and the predicts a scale and shift invarient depth map for each segment. Finally their model stiches each local depth segment by predicting its scale and shift based on the global context of the image.

\textbf{Edge Refinement}
Ramamonjisoa et. al. \cite{Ramamonjisoa_2020_CVPR} tried to train a 'depth displacement field' network to fix the occlusion boundary locations in the an already given depth estimation. \mahdi{I think we should evaluate against them since they are also doing some kind of depth refinement emphasizing edges and occlusion boundaries.}
Tian and Li \cite{tian2016color} propose to use the color image as a guide for properly aligning edges in depth maps and fill in resulting holes via interpolation.
A similar procedure is also suggested by Sato and Kimura \cite{sato2020simple}. Dziembowski et. al. \cite{dziembowski2016depth} also use the RGB image as a guide and a Bilateral Filter to enhance low resolution depth maps. Hong et al.\cite{hong2016depth} also introduce an image-guided edge refinement approach, which is based on superpixels.

Rossi et al. \cite{rossi2020joint} work with the assumption that most human-made structures are based on planes and most other shapes can be approximated as such. They suggest a graph-based solver to refine depth estimations by finding an optimal set of planes attached to the depth values.
\SD{ToDo: test against this.}

\paragraph{Patch-based Image Editing}
Darabi et. al. \cite{darabi2012image} use image patches to merge inconsistent images. They use a Screened Poisson Solver, which did not work in our case. Additionally, they introduce a mixed $L_2$- $L_0$ norm to keep sharpness. \SD{We should test our merging network against this}

Yu et al. \cite{yu2020high} introduce a crop-based approach for high resolution image matting. While their idea is similar to ours, their method is specifically designed for image matting scenarios and thus not applicable in our case.




==> tex/results_orig.tex <==
% !TEX root = ../depth.tex

Results.

\subsection{Training}
\label{sec:Training}
 We train our merging network for \SD{add epochs} epochs on a \SD{add hardware specification}. We upscale the existing datasets IBIMS-1, Middleburry2014 and TAU to create a pseudo-HD dataset for training. \LM{Why ibims1? Are we using its ground-truth depth maps?}  Using the lower and upper bound from double estimation individually, we create input pairs of low- and high-frequency depth estimation.
 We found that matching the depth distribution of the ground truth with the distribution generated by a depth estimation network is key.\SD{todo: explain why original GT won't work} Instead of using the original ground truth from the datasets directly, we create a single estimation with the "optimal" in-between resolution described in section \ref{sec: double est}, since this best approximates our target.  
%\input{images/refinement}
\subsection{Experiments}
\label{sec:experiments}

\subsection{Evaluation}
\input{images/doubleest}
\input{images/stateoftheart}


\paragraph{Metric}
\paragraph{Comparison against original MiDas}
\paragraph {Comparison against MiDas+}
\paragraph{Comparison against other refinement methods}
\begin{itemize}
    \item Bilateral filter
    \item Edge of Depth
    \item Displacement Fields
    \item Feature upscaling
\end{itemize}
\paragraph{extension to other depth estimation networks}
\begin{itemize}
    \item Megadepth
    \item SGR
\end{itemize}
\paragraph{Discussion on other metrics, ground truth issues etc}
\begin{itemize}
    \item Middleburry 2014 dataset:\cite{Scharstein2014HighResolutionSD}
    \item IBIMS-1 dataset: \cite{Koch18}
    \item TAU dataset: \cite{haim2018depth}
    \item little high-resolution depth ground truth available. Biggest resolution to our knowledge currently: Middleburry 2014 (roughly 6MP).
    \item ground truth data rarely perfect:
    gaps, large interpolated areas for Kinect data, quantization artifacts
    \item ground truth depth often imperfect at edges, which is exactly the areas we're interested in.
    \item MSE and generally global metrics are not reliable in our case since they can't reflect the accuracy of details. 
   
\end{itemize}



\subsection{Ablation study}
\input{imagetex/oraclemidas}
\begin{itemize}
    \item impact of input size for MiDas
    \item impact of crop size/ context
    \item impact of upscaling/downscaling
    \item impact of stride size
    \SD{ToDo: conduct more experiments to find perfect stride}
    \item minimum/maximum image resolution
\end{itemize}

\subsection{Extension to other applications}

